PID: Prompt-Independent Data Protection Against Latent Diffusion Models

The few-shot fine-tuning of Latent Diffusion Models (LDMs) has enabled them to grasp new concepts from a limited number of images. However, given the vast amount of personal images accessible online, this capability raises critical concerns about civil privacy. While several previous defense methods have been developed to prevent such misuse of LDMs, they typically assume that the textual prompts used by data protectors exactly match those employed by data exploiters. In this paper, we first empirically demonstrate that breaking this assumption, i.e., in cases where discrepancies exist between the textual conditions used by protectors and exploiters, could substantially reduce the effectiveness of these defenses. Furthermore, considering the visual encoder's independence from textual prompts, we delve into the visual encoder and thoroughly investigate how manipulating the visual encoder affects the few-shot fine-tuning process of LDMs. Drawing on these insights, we propose a simple yet effective method called \textbf{Prompt-Independent Defense (PID)} to safeguard privacy against LDMs. We show that PID can act as a strong privacy shield on its own while requiring significantly less computational power. We believe our studies, along with the comprehensive understanding and new defense method, provide a notable advance toward reliable data protection against LDMs.

==> temp.tex <==


(0) Select data
we randomly select 10 celebrities and choose 4 images for each.


(1) Protect image 
For defense, we set the prompt $\bm{c_{prot}}$ as \textit{A photo of sks person}. (And we protect the images with the ASPL and FSGM algorithm, using the $c_{prot}.)


(2) Fine-tuning
For each one of the selected 10 celebrities, we fine-tune the model using three prompts $\bm{c_{explo}}$, obtaining 30 different fine-tuned models. 


(3) Generate Image
For each LDM, we generate 20 images with the 3 prompts respectively {A photo of sks person, A selfie of sks person, A DSLR portrait of sks person}. 


(4) Evaluate
Then we evaluate each set of the images with the four metrics that we defined. 


(5) Get Results
Lastly, for the three models belonging to each instance, we select the model that generates the sets of images having the highest FDS to represent the defenses' performance for this instance in the $c_{prot} \neq c_{explo}$ case. 



    

